Foundations for a Probabilistic Event Calculus

We present PEC, an Event Calculus (EC) style action language for reasoning about probabilistic causal and narrative information. It has an action language style syntax similar to that of the EC variant Modular-E. Its semantics is given in terms of possible worlds which constitute possible evolutions of the domain, and builds on that of EFEC, an epistemic extension of EC. We also describe an ASP implementation of PEC and show the sense in which this is sound and complete.

==> Sections/5implementation.tex <==
% Nobody currently editing

\section{ASP Implementation and Evaluation}

We have implemented PEC for the class of domains in which the bodies of c-propositions $\theta$ are conjunctive formulas. The implementation and example domain descriptions can be found at \url{http://github.com/dasaro/pec}.
An overview of the implementation is given in the following diagram:

\vspace{-1.2em}

	\begin{center}
		\begin{tikzpicture}[>=latex',special node/.style={draw,minimum height=2cm,inner sep=0.5em,outer sep=0.5em,rounded corners,align=center,text width=2cm}]
		\node [special node] (Translator) {\small \textbf{Translator} \\ (Flex and Bison) };
		\node [special node,right=2cm of Translator] (Clingo) {\small \textbf{Grounder and Solver} \\ (Clingo)};
		\node [special node,right=2cm of Clingo] (AWK) {\small \textbf{Text processing} \\ (AWK)};
		
		\coordinate[above=1cm of Translator] (Input);
		\coordinate[above=1cm of Clingo] (Query);
		\coordinate[above=1cm of AWK] (Output);
		
		\draw [->] (Translator) -- node[above,midway] {\small translatedD.lp} (Clingo);
		\draw [->] (Clingo) -- node[above,align=center,text width=2cm] {\small traces as \\stable models} (AWK);
		n
		\draw [->] (Input) -- node[right,midway,text width=2cm] {\small inputD.pec} (Translator);
		\draw [->] (Query) -- node[right,midway,text width=2cm] {\small pec.lp \\ query.lp} (Clingo);
		\draw [->] (AWK) -- node[right,midway,text width=2cm] {\small answer} (Output);
		\end{tikzpicture}
	\end{center}

We developed a translator which turns a PEC domain description $ \mathcal{D} $ into an ASP program, using the lexical analyser Flex and the parser generator Bison (see e.g. \cite{levine2009flexbison}). The output of the translator together with an ASP formulation of the domain-independent part of the semantics and a query\footnote{We have not yet implemented a mechanism for translating arbitrary h-propositions to ASP programs. This is planned for future work.} are then processed by Clingo (see e.g. \cite{gebser2014clingo}). This returns answer sets, each of which represents a trace and the corresponding well-behaved world w.r.t. $ \mathcal{D} $. A standard text processing tool, AWK (see e.g. \cite{aho1987awk}) then processes the resulting answer sets and calculates the probability associated with the given query using Equation \eqref{eq:extendedmodel}.
